Response Selection for Multi-Party Conversations with Dynamic Topic Tracking

While participants in a multi-party multi-turn conversation simultaneously engage in multiple conversation topics, existing response selection methods are developed mainly focusing on a two-party single-conversation scenario. Hence, the prolongation and transition of conversation topics are ignored by current methods. In this work, we frame response selection as a dynamic topic tracking task to match the topic between the response and relevant conversation context. With this new formulation, we propose a novel multi-task learning framework that supports efficient encoding through large pretrained models with only two utterances at once to perform dynamic topic disentanglement and response selection. We also propose Topic-BERT an essential pretraining step to embed topic information into BERT with self-supervised learning. Experimental results on the DSTC-8 Ubuntu IRC dataset show state-of-the-art results in response selection and topic disentanglement tasks outperforming existing methods by a good margin.

==> Content/conclusion.tex <==
This paper describes our model that are evaluated on 3
sub-tasks of Track 2 of DSTC-8. Pre-trained attention-based
network for multi-turn dialogue systems are designed for
each sub-task according to different evaluation dimensions.
We find that the context retrieval is a very direct and effective way to remove contextual noise. We adapt data augment method to make soft topic modeling possible, the sentence-sentence topic relationship is also quite helpful in downstream topic prediction and response selection tasks. We adapt pre-training strategy with MLM and NSP with topic information, then the topic information could be used to act as attention query to fuse the contextual vectors with topic attention. Lastly, we jointly train topic prediction,response selection and disentanglement to get a significant improvement of the final result. In future, unsupervised topic modeling could be used as topic cluster to model the latent representation of conversation topic, this new dimension of view will make the response selection and generation more effective.

==> Content/experiment_revise.tex <==
In this section, we present our experiments, including the datasets, experimental setup, evaluation metrics, and the results with analysis.

\subsection{Dataset}
Considering our setting, a public available Ubuntu dataset in DSTC-8\cite{kim2019eighth} is suitable for our problem setting. Ubuntu Task 1 dataset is a single-topic multi-party dialogue setting which is considered for our topic prediction and the test set contains 1 positive response and 4 randomly selected negative responses out of 99 for each testing instance. Ubuntu Task 2 dataset is a long Ubuntu chat log with multi-party conversations on-going simultaneously which is used for our response selection and the test set contains 1 positive response and 99 negative responses for each testing instance. Ubuntu Task 4 dataset is formed by multi-party conversations with link annotations, where each instance has 1500 utterances with around 500 annotation links. In addition, Ubuntu V1 \cite{lowe2015ubuntu} with 1M train set, 500K validation and 500K was 

\subsection{Experimental Setup}
\label{BERT topic pairs}
We adopt the vanilla pretrained uncased BERT-Base (which has 12 layers with a hidden size of 768, provided by hugging face library) \footnote{\url{https://github.com/huggingface/transformers}} as our input-encoder, we initialised our BERT weights with uncased BERT-Base configuration. In addition, according to the methodology we discussed in section \ref{Self-supervised BERT Pretraining}, we obtained 13561221 train sentence pairs, 576414 validation sentence pairs Task 1 corresponding dataset. Inspired by \cite{gu2020pre,BERT-enhance}, we post trained our input-encoder (uncased BERT-Base) 10 epochs more with augmented train and validation topic sentence pairs and the batch size is set to 96 with maximum 10 utterance pairs. Then 2 more epochs with test topic sentence pairs was used for finetuning.  We used cross-entropy loss and Adam optimizer with a learning rate of 2e-5 and a linear decay schedule with warm-up 0.1. Regarding some hyper-parameters, the maximum sequence length of the concatenation of a context-response pair was set to 192 (96 for response), and the ratio of dropout is 0.1 to prevent over-fitting. The evaluation metric is the average of accuracy, precision and recall. Then, linear feed-forward layer layer with a hidden size of 768$\times$2 to reduce it from vector to scalar for downstream tasks (weights are not shared).

\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{1}
{\begin{tabular}{c|ccc}
\toprule
%\textbf{Task}& \multicolumn{3}{|c}{\textbf{Data} } \\
%\midrule
Task & Train set & Validation set & Test set  \\
 \midrule
 Task 1& 225,367 & 4,827 & 5,529 \\
 Task 2& 112,262 & 9,565 & 9,027 \\
%\midrule
 Task 4 &153&10&10 \\
\bottomrule
\end{tabular}}
\caption{DSTC-8 Ubuntu Dataset Statistics}
\label{table:data}
\end{table}
For response selection, the candidate pool may not contain the correct response, so we need to choose a threshold. When the probability of positive labels was smaller than the threshold, we predicted that candidate pool did not contain the correct response. The threshold was selected from the range [0.7, 0.75, .., 0.95]\cite{gu2020pre}, based on the validation set, it was set to 0.90 finally. We used the validation set to set the stop condition to select the best model for testing. 

\subsection{Evaluation Metrics}
Track 2 considered a range of metrics
when comparing models. Following \cite{lowe2015ubuntu}, the
Recall@N is used for topic prediction and response selection, which counts how
often the correct answer is within the top N specified by the model. The values of N can be 1, 5, and 10. In addition, the Mean Reciprocal Rank (MRR) is also considered which is a widely used metric from the ranking literature. In the final comparison, the mean of Recall@10 and MRR is used. 

For disentanglement, exact match F-1 calculated using the number of perfectly matching conversations, excluding conversations with only one message. For topic prediction, we simply use precision, recall and F-1 metrics

\subsection{Baseline Models}
\subsubsection{Response Selection}
\label{RS}
We compare the proposed Topic-BERT approach with several existing and state-of-the-art approaches for response selection:
\begin{itemize}
\item\textbf{BERT.} The vanilla pretrained uncased BERT-Base\footnote{\url{https://github.com/huggingface/transformers}} was the base model. We follow \cite{gu2020pre} to posttrain BERT-Base on task 1 dataset with 10 more epochs for response selection and topic prediction with batch size of 16. The initial learning rate was set to 2e-5. The maximum sequence length of the concatenation of a context-response pair was set to 512. In finetuning, 2 more epoch was used for response selection on task 2 dataset. Adam optimizer with a learning rate of 2e-5 and a linear decay schedule with warm-up 0.06 was selected.  

\item\textbf{ToD-BERT.} ToD-BERT \cite{wu2020tod} is a pre-trained language model with 9 task-oriented dialogue datasets, it surpasses BERT in downstream response selection task. We compare our topic pre-trained BERT with the ToD-BERT in topic prediction, response selection and disentanglement.

\item\textbf{BERT-ESIM.} Model ensembling of ESIM and BERT with gradient boosting classifier which rank as the second team in DSTC-8 response selection \cite{BERT-ESIM}.

\item\textbf{Adapt-BERT.} BERT model with task-related pretraining and context modeling through hard and soft context modeling which rank as the top-1 team in DSTC-8 response selection challenge \cite{BERT-enhance}.
\end{itemize}

\subsubsection{Topic Prediction}
\label{BERT TP}
\begin{itemize}
\item\textbf{BERT.} We use our post trained BERT which is discussed in \ref{BERT topic pairs} as our BERT baseline for topic prediction.
\item\textbf{ToD-BERT.} We initialise BERT model with ToD-BERT and finetune it with our obtained topic sentences pairs \ref{Self-supervised BERT Pretraining} as our ToD-BERT baseline for topic prediction.
\end{itemize}
\subsubsection{Disentanglement}
We use our finetuned \textbf{BERT} and \textbf{ToD-BERT} model mentioned in \ref{BERT TP} as our baselines by taking the context utterance-response pairs from a dialogue as inputs, in addition，a single-layer BiLSTM with hidden size of 384 (BiLSTM output hidden size will be 768 to match with BERT output hidden size) is employed on top of the outputs of BERT [cls] outputs to capture the semantics across different messages which are denoted as and a single layer feedforward neural network with 768 $\times$ 4 hidden units will be the classifier.
\begin{itemize}
\item\textbf{Feed-Forward.} We use the feed-forward model from \cite{acl19disentangle} as the baseline model. In DSTC-8, \citet{acl19disentangle} provided a fully trained model.\footnote{\url{https://github.com/dstc8-track2/NOESIS-II/tree/master/subtask4}} The provided model is trained using a two-layer neural network. The input is 77 hand engineered features combined with word average embeddings from pre-trained Glove embeddings. 
\item\textbf{Masked Hierarchical (MH) BERT.} It is a two stage BERT to model the conversation structure where the low level BERT is to capture the utterance-level contextual representation between utterances. And the high level BERT is to modeling the conversation structure with an ancestor masking approach to avoid irrelevant connections \cite{zhu2019did}. 
\end{itemize}

\subsection{Experiment Result}
Table~\ref{table:response selection} presents the evaluation results of our methods on the response selection task. Table~\ref{table:topic prediction} shows the evaluation results of our methods on the topic prediction task.
And Table~\ref{table:disentanglement} presents the evaluation results of our methods on the disentanglement task.

From Table~\ref{table:response selection}, we can see that our context filtering, self-supervised topic training and topic attention contribute positively to our model, the metric of Recall@1 improved from 0.298 (BERT) to 0.696 (Topic BERT with standalone response selection), which shows pre-training BERT with task related data can improve BERT model in response selection task.Furthermore, the performance continues to increase from 0.696 to 0.710 when we jointly train response selection and topic prediction, it shows an effective utilization of topic information in selecting response to outperform Adapt-BERT which is the current state-of-the-art performance in DSTC-8 response selection task \cite{kim2019eighth}. Then we replace topic prediction with disentanglement, the performance further improved from 0.710 to 0.720, which shows response selection can utilize topic tracing by sharing the link relationship of utterances. Finally, our multi-task model with topic prediction, disentanglement and response selection achieve a better result comparing to the baselines.

Meanwhile, From Table~\ref{table:response selection},\ref{table:topic prediction},\ref{table:disentanglement}, we can see that our pre-training with topic sentence pairs data is more effective than BERT pre-training with dialogue data. Our post train strategy leverage utterance-utterance topic relationship which makes sentence level encoding simpler and effective.

\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.85}
{\begin{tabular}{l|cccc}
\toprule
%Model& \multicolumn{4}{|c}{\textbf{Result} } \\
%\midrule
Model & Recall@1 & Recall@5 & Recall@10 & MRR  \\
\midrule
\hline
BERT & 0.298 & 0.513 & 0.589 & 0.377\\
ToD-BERT & 0.588 & 0.823 & 0.885 & 0.691 \\
%ToD-BERT & 0.588 & 0.823 & 0.885 & 0.691 \\
BERT-ESIM & 0.596 & 0.847 & 0.904 & 0.707 \\
Adapt-BERT & 0.706 & 0.916 & 0.957 & 0.799\\\hline
Topic-BERT & {\bf 0.726} & {\bf 0.930} & {\bf 0.970} & {\bf 0.807} \\
\textminus TP & 0.720 & 0.927 & 0.964 & 0.803  \\
%Response Selection (*) & 0.614 & 0.855 & 0.891 & 0.724 \\
%\midrule
\textminus D & 0.710 & 0.924 & 0.960 & 0.800 \\
%Response Selection + Topic Prediction (*) & 0.628 & 0.872 & 0.904 & 0.732 \\
%\midrule
\textminus TP \textminus D & 0.696 & 0.910 & 0.950 & 0.790 \\\hline
%Response Selection + Disentanglement (*) & 0.633 & 0.875 & 0.906 & 0.734  \\
%\midrule
%Response Selection + Topic Prediction + Disentanglement (*) &0.639 & 0.880 & 0.912 & 0.739 \\
%\bottomrule
%\hline

\end{tabular}}
\caption{Response selection result with our pre-trained Topic BERT. ``RS" indicates our model architecture with response selection task, ``TP" indicates our model architecture with topic prediction task and ``D" indicates our model architecture with topic disentanglement task. }
\label{table:response selection}
\end{table}


\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{1}
{\begin{tabular}{l|ccc}
\toprule
%Model& \multicolumn{3}{|c}{\textbf{Result} } \\
%\midrule
Model &Precision & Recall & F-1   \\
\midrule
\hline
BERT & 0.523 & 0.482 & 0.502 \\
ToD-BERT & 0.626 & 0.563 & 0.593\\\hline
Topic-BERT & {\bf 0.890} & {\bf 0.847} & {\bf 0.868} \\
\; w/o FT & 0.848 & 0.781 & 0.813 \\
\textminus D & 0.891 & 0.845 & 0.867 \\
\textminus RS &  0.889 & 0.840 & 0.864 \\
\textminus D \textminus RS & 0.866 & 0.793 & 0.828  \\
%+ TP& 0.866 & 0.793 & 0.828  \\
%+ TP + RS & 0.891 & 0.845 & 0.867 \\
%+ TP + D & 0.889 & 0.840 & 0.864  \\
%Topic Prediction (*) & 0.663 & 0.615 & 0.638  \\
%\midrule
%Topic Prediction + Response Selection (*) & 0.694 & 0.653 & 0.673 \\
%\midrule
%Topic Prediction + Disentanglement (*) & 0.701 & 0.660 & 0.680  \\
%\midrule
%Response Selection + Topic Prediction + Disentanglement (*) &0.708 & 0.675 & 0.691 \\
\bottomrule
%\hline
%Our Topic BERT & 0.848 & 0.781 & 0.813 \\
%ToD-BERT & 0.626 & 0.563 & 0.593 \\
\end{tabular}}
\caption{Topic prediction result with our pre-trained Topic BERT. ``RS" indicates our model architecture with Response Selection task, ``TP" indicates our model architecture with Topic Prediction task and ``D" indicates our model architecture with topic Disentanglement task.}
\label{table:topic prediction}
\end{table}

\if 0 
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{1}
{\begin{tabular}{l|ccc}
\toprule
Model& \multicolumn{3}{|c}{\textbf{Result} } \\
%\midrule
&Precision & Recall & F-1   \\
\midrule
\hline
TP& 0.866 & 0.793 & 0.828  \\
%Topic Prediction (*) & 0.663 & 0.615 & 0.638  \\
%\midrule
+ RS & 0.891 & 0.845 & 0.867 \\
%Topic Prediction + Response Selection (*) & 0.694 & 0.653 & 0.673 \\
%\midrule
+ D& 0.889 & 0.840 & 0.864  \\
%Topic Prediction + Disentanglement (*) & 0.701 & 0.660 & 0.680  \\
\midrule
RS + TP + D &0.890 & 0.847 & 0.868 \\
%Response Selection + Topic Prediction + Disentanglement (*) &0.708 & 0.675 & 0.691 \\
\bottomrule
\hline
Our Topic BERT & 0.848 & 0.781 & 0.813 \\
BERT & 0.523 & 0.482 & 0.502 \\
%ToD-BERT & 0.626 & 0.563 & 0.593 \\
\end{tabular}}
\caption{Topic prediction result with our pre-trained Topic BERT. ``RS" indicates our model architecture with Response Selection task, ``TP" indicates our model architecture with Topic Prediction task and ``D" indicates our model architecture with topic Disentanglement task.}
\label{table:topic prediction}
\end{table}

\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{1}
{\begin{tabular}{l|ccc}
\toprule
Model& \multicolumn{3}{|c}{\textbf{Result} } \\
%\midrule
&Precision & Recall & F-1   \\
\midrule
\hline
D& 0.689 & 0.678 & 0.683  \\
%Disentanglement (*) & 0.612 & 0.603 & 0.607  \\
%\midrule
+ TP & 0.705 & 0.692 & 0.698 \\
%Disentanglement + Topic Prediction (*) & 0.635 & 0.627 & 0.631 \\
%\midrule
+ RS & 0.749 & 0.727 & 0.737  \\
%Disentanglement + Response Selection (*) & 0.643 & 0.622 & 0.632  \\
\midrule
RS + TP + D &0.754 & 0.725 & 0.739\\
%Response Selection + Topic Prediction + Disentanglement (*) &0.647 & 0.630 & 0.638 \\
\bottomrule
\hline
Feed-Forward & 0.748 & 0.718 & 0.733 \\
\end{tabular}}
\caption{Topic disentanglement result with our pre-trained Topic BERT. ``RS" indicates our model architecture with response selection task, ``TP" indicates our model architecture with topic prediction task and ``D" indicates our model architecture with topic disentanglement task.}
\label{table:disentanglement}
\end{table}
\fi

\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{1}
{\begin{tabular}{l|ccc}
\toprule
%Model& \multicolumn{3}{|c}{\textbf{Result} } \\
%\midrule
Model & Precision & Recall & F-1   \\
\midrule
\hline
BERT & 0.431 & 0.417 & 0.424  \\
MH BERT & 0.539 & 0.517 & 0.528\\
ToD-BERT & 0.612 & 0.603 & 0.607\\
Feed-Forward & 0.748 & 0.718 & 0.733 \\\hline
Topic-BERT & {\bf 0.754} & {\bf 0.725} & {\bf 0.739}\\
\textminus TP & 0.749 & 0.727 & 0.737  \\
%+ D& 0.689 & 0.678 & 0.683  \\
%Disentanglement (*) & 0.612 & 0.603 & 0.607  \\
%\midrule
\textminus RS & 0.705 & 0.692 & 0.698 \\
%+ D + TP & 0.705 & 0.692 & 0.698 \\
%Disentanglement + Topic Prediction (*) & 0.635 & 0.627 & 0.631 \\
%\midrule
\textminus TP \textminus RS& 0.689 & 0.678 & 0.683  \\
%+ D + RS & 0.749 & 0.727 & 0.737  \\
%Disentanglement + Response Selection (*) & 0.643 & 0.622 & 0.632  \\
%\midrule
%Response Selection + Topic Prediction + Disentanglement (*) &0.647 & 0.630 & 0.638 \\
\bottomrule
%\hline
\end{tabular}}
\caption{Topic disentanglement result with our pre-trained Topic BERT. RS indicates our model architecture with response selection task, TP indicates our model architecture with topic prediction task and D indicates our model architecture with topic disentanglement task.}
\label{table:disentanglement}
\end{table}

\if 0
%move to appendix
\begin{table*}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.8}
{\begin{tabular}{c|c}
\toprule
\textbf{Speaker}& \textbf{Utterance}  \\
 \midrule
 None & None \\
 None & None \\
 participant\_23 & [n=olid@ACC9C91A.ipt.aol.com] has joined #ubuntu \\
 participant\_25 & i would just like to know, how can i found out the support webcams for dapper? \\
 participant\_23 & in sessions what do i have to add to the start of my command to run the command as root when i boot up ? \\
 participant\_25 & *supported \\
 participant\_23 & \textbf{to start lampp} \\
 participant\_23 & \textbf{opt/lampp/lampp start} \\
 participant\_25 & is there a command in shell, or a section in the ubuntu website to find out all the supported webcams for dapper drake? \\
 participant\_23 & ok ty participant\_20\\
\midrule
ToD-BERT & participant\_25 , permission on /home/luigi/wwwebserver http://pastebin.ubuntu.com/75435/ \\
Topic-BERT & \textbf{ill put it in rc.local}\\
Ground-truth & ill put it in rc.local\\
 \bottomrule
\end{tabular}}
\caption{Top-1 response selection performance comparison}
\label{table:example}
\end{table*}
\fi

Similarly, the result in Table~\ref{table:topic prediction} also shows our topic attention enhance the topic matching of two utterances in the metric of F-1 by 1.5\%. Response selection and disentanglement shows an equivalent effect on topic prediction in multi-task setting which shows contextual and link relationship can help topic prediction. 

In addition, from the result shown in Table~\ref{table:disentanglement}, we can see that the multi-task setting enrich the link relationship together with topic prediction and response selection, the highly related tasks make our model outperform the baseline feed forward network with hand-crafted features. Meanwhile, due to the self-links in disentanglement not existing in topic prediction and response selection. It beats the SOTA baseline marginally.

\if 0 
Table~\ref{table:example} shows our qualitative comparison. Our topic pre-training strategy could retrieve response based on topic relevance, those informative non-topic relevant utterances will not influence our response selection.
\fi




==> Content/introduction_revise.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[scale= .4]{image/running-example-crop.pdf}
    \caption{Ubuntu IRC log example, utterances from top to bottom are following a time-sequence, earliest text comes first. Curved arrow shows the link annotation which is pointing at its parent utterance.Here, the color of the utterances represents conversation topic and the same color indicates the utterances are from a same conversation group.}
    \label{fig:dialogue example}
\end{figure}

%In the recent years, the progress of task-oriented dialogue system is significant. They assist people in real-world business such as booking system to complete a specific task through interaction with natural language \cite{Trung-2006}. One well-known task-oriented dialogue system is response selection which is a retrieval-based dialogue system to predict a suitable response from a pool of response candidates.
In recent years, with the influx of deep learning methods in natural language processing (NLP), there has been a lot of interests in building effective task-oriented dialogue systems that can assist people in real-world business such as booking tickets, ordering food and solving technical issues \cite{Trung-2006}. \textbf{Retrieval-based} response generation that selects a suitable response from a pool of candidates (pre-existing human responses) has become a popular approach to framing dialog. Compared to the \textbf{generation-based} systems that \emph{generates} new utterances, retrieval-based systems produce fluent, grammatical and informative responses, and have been widely adopted in commercial dialogue systems \cite{GaoconvAI,gunasekara2019dstc7,weston2018retrieve,henderson2019convert}.

The primary researches \cite{gandhe2010ve,Lowe2017TrainingED} have demonstrated the potential of response selection in a practical dialogue system. Moreover, early studies focused on single-turn conversations, where only the last input utterance is considered as the context query \cite{1-turn,10.1145/2911451.2911542}.   

achieves an success in single-turn response selection system \cite{1-turn}. However, there is a need beyond two-agent conversation modeling, a form of multi-speaker, multi-turn dialogue is necessary for a real-world task-oriented response selection system \cite{lowe2015ubuntu,Lowe2017TrainingED}. Similar to single-turn response selection systems, most of previous works \cite{Lowe2017TrainingED,zhou2016multi,ESIM2} use the entire historical utterance as one turn to represent the context to simplify the multi-turn response selection task to a sing-turn problem. Meanwhile, some studies \cite{IMN,SMN,DAM} also shows an effective approach to enhance utterance-response matching information with various attention mechanism \cite{bahdanau2014neural}. The aforementioned methods works well for a detached or disentangled conversation, however there are several interlocutors communicate with each other in a real-world case, such as Internet Relay Chat (IRC) \cite{Kummerfeld2019ALC}, multiple conversations are on-going simultaneously. 

Figure~\ref{fig:dialogue example} shows a real-world dialogue example, the speaker \emph{Nafallo} participate in 3 topics of conversations which are highlighted by different color. The complex contextual information make response selection less accurate for existing methods. By contrast, a proper response should match with its context in terms of the same topic. Non-relevant topic context should not be the reason to influence the selected response. Therefore, similar topic disentangled context should point to similar response.

Recently, pre-trained language model BERT is widely applied in response selection task \cite{BERT,vig2019comparison,BERT-SM}. They often pre-train BERT with domain specific data to learn a contextual representation for downstream tasks. They have shown speaker-embedding \cite{BERT-SM}, self-supervised pre-training and contextual filtering \cite{BERT-enhance} could improve the response selection performance. However, the topic of conversation still not emphasized by these methods and huge amount of turns make it worse.

In this paper, we propose a BERT-based framework for response selection task. Considering the correlation between multi-turn response selection and contextual topic disentanglement. We encode the context utterance and response pair and feed them into BERT. In order to model the topic relationship, we pre-train our BERT model with topic related sentence pairs instead of the whole context-response pairs to incorporate a soft representation of topic dynamics with 2 training objectives which are Masked Language Modeling (MLM) and Next Sentence Prediction (NSP). The topic related sentence pairs are generated from the given dialogue, there will be no extra cost for data collection. In addition, we use topic attention and self-attention to leverage topic dynamics in downstream response selection task. Inspired by the connection between response selection and topic-disentanglement, topic prediction and topic disentanglement are two derivative tasks that our model will target on.

In summary, we have made several contributions which are:
\begin{itemize}
  \item Self-supervised approach to model utterance-utterance topic relationship which are represented as hidden state vectors that dynamically change with time steps in the dynamic modeling. The BERT encoded topic vector will be further utilized to enhance downstream response selection with attention mechanism. 
  \item Multi-task learning of response selection by sharing neural network hidden representation to encode the sentences for both topic prediction, response selection and topic disentanglement.  
\end{itemize}


    

